Stable Diffusion-based Data Augmentation for Federated Learning with Non-IID Data

The proliferation of edge devices has brought Federated Learning (FL) to the forefront as a promising paradigm for decentralized and collaborative model training while preserving the privacy of clients' data. However, FL struggles with a significant performance reduction and poor convergence when confronted with Non-Independent and Identically Distributed (Non-IID) data distributions among participating clients. While previous efforts, such as client drift mitigation and advanced server-side model fusion techniques, have shown some success in addressing this challenge, they often overlook the root cause of the performance reduction - the absence of identical data accurately mirroring the global data distribution among clients. In this paper, we introduce Gen-FedSD, a novel approach that harnesses the powerful capability of state-of-the-art text-to-image foundation models to bridge the significant Non-IID performance gaps in FL. In Gen-FedSD, each client constructs textual prompts for each class label and leverages an off-the-shelf state-of-the-art pre-trained Stable Diffusion model to synthesize high-quality data samples. The generated synthetic data is tailored to each client's unique local data gaps and distribution disparities, effectively making the final augmented local data IID. Through extensive experimentation, we demonstrate that Gen-FedSD achieves state-of-the-art performance and significant communication cost savings across various datasets and Non-IID settings.

==> algorithms.tex <==
\section{Algorithms}


\begin{algorithm}[H]
\caption{Federated Learning}
\label{alg:FedAvg}

% \DontPrintSemicolon
% \SetCommentSty{mycommfont}
% \SetAlgoLined
% \SetKwInOut{Req}{Require}
% \SetKwFunction{FClient}{ClientUpdate}
% \SetKwProg{Fn}{}{:}{}

\begin{algorithmic}[1]
\REQUIRE number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$).
%\SetKwProg{Fn}{Server Executes}{:}{}
\STATE \textbf{Server Executes:}
\STATE Initialize the server model with $\btheta_g^0$ \;
\FOR {each round $t = 0, 1, \ldots, T-1$}
\STATE $m \leftarrow {\rm{max}}(C \cdot N,1)$ \;
\STATE $S_t \leftarrow $(random set of m clients) \; %\tcp*{set of $m$ available clients}
\FOR {each client $k \in S_t$ \rm{\textbf{in parallel}}}
\STATE $\btheta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \btheta^t_{g} )$ \; 
%$\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
\ENDFOR
\STATE $\btheta^{t+1}_{g}=\mathtt{ModelFusion}(\{\btheta_k \}_{k \in S_t})$
\ENDFOR
\vspace{1mm}
\FUNCTION {$\mathtt{ClientUpdate}(k, \btheta^t_{g})$}
\STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
\STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k^{train}$ into batches of Size $B$})\;
\FOR {each local epoch $ \in \{1, \ldots, E\}$}
\FOR {each batch $\mathbf{b} \in \mathcal{B}$}
\STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} \ell(f_k(\bx; \btheta^{t}_k), y)$\;
\ENDFOR
\ENDFOR
\STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
\ENDFUNCTION
% \Fn{\FClient{$k, \btheta^t_{g}$}}{
%     \STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
%     \STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
%     \For {each local epoch $i = 1, \dots, E$} {
%         \For {each batch $\mathbf{b} \in \mathcal{B}$} {
%             \STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} f_k(\btheta^{t}_k; \mathbf{b})$\;
%         }
%     }
%     \STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
%     \KwRet $\btheta^{t+1}_{k}$\;
% }
\end{algorithmic}
\end{algorithm}


% \begin{algorithm}[H]
% \caption{FedAvg}
% \label{alg:FedAvg}

% % \DontPrintSemicolon
% % \SetCommentSty{mycommfont}
% % \SetAlgoLined
% % \SetKwInOut{Req}{Require}
% % \SetKwFunction{FClient}{ClientUpdate}
% % \SetKwProg{Fn}{}{:}{}

% \begin{algorithmic}[1]
% \STATE \textbf{Require:} number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$).
% %\SetKwProg{Fn}{Server Executes}{:}{}
% \STATE \textbf{Server Executes:}
% \STATE $\quad$ Initialize the server model with $\btheta_g^0$ \;
% \FOR {each round $t = 0, 1, \dots, T-1$}
% \STATE $\quad$ $m \leftarrow {\rm{max}}(C \cdot N,1)$ \;
% \STATE $\quad$ $S_t \leftarrow $(random set of m clients) \; %\tcp*{set of $m$ available clients}
% $\quad$ \FOR {each client $k \in S_t$ \rm{\textbf{in parallel}}}
% \STATE $\quad$ $\btheta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \btheta^t_{g} )$ \; 
% %$\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
% \ENDFOR
% \STATE $\quad$ $\btheta^{t+1}_{g}=\mathtt{ModelFusion}(\{\btheta_k \}_{k \in S_t})$
% \ENDFOR
% \vspace{1mm}
% \FUNCTION {$\mathtt{ClientUpdate}(k, \btheta^t_{g})$}
% \STATE H
% \ENDFUNCTION
% % \Fn{\FClient{$k, \btheta^t_{g}$}}{
% %     \STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
% %     \STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
% %     \For {each local epoch $i = 1, \dots, E$} {
% %         \For {each batch $\mathbf{b} \in \mathcal{B}$} {
% %             \STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} f_k(\btheta^{t}_k; \mathbf{b})$\;
% %         }
% %     }
% %     \STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
% %     \KwRet $\btheta^{t+1}_{k}$\;
% % }
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \caption{FedProx}
% \label{alg:FedProx}

% \DontPrintSemicolon
% \SetCommentSty{mycommfont}
% \SetAlgoLined
% \SetKwInOut{Req}{Require}
% \SetKwFunction{FClient}{ClientUpdate}

% \Req{number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), 
% local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$), FedProx parameter ($\mu$)\;}
% \SetKwProg{Fn}{Server Executes}{:}{}
% \Fn{}{
% Initialize the server model with $\theta_g^0$ \;
% \For {each round $t = 0, 1, \dots, T-1$} {
%  $m \leftarrow {\rm{max}}(C \cdot N,1)$\;
%  $S_t \leftarrow $(random set of m clients)\; %\tcp*{set of $m$ available clients}
% \For  {each client $k \in S_t$ \rm{\textbf{in parallel}}}
% { 
% $\theta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \theta^t_{g} )$ \; 
% }

% $\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
% }
% }
% %\Indm
% \SetKwProg{Fn}{}{:}{}
% \Fn{\FClient{$k, \theta^t_{g}$}}{
%      $\theta^{t}_k \leftarrow \theta^t_{g}$\;
%      $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
%     \For {each local epoch $i = 1, \dots, E$} {
%         \For {each batch $\mathbf{b} \in \mathcal{B}$} 
%         {
%              $\theta^{t+1}_k \leftarrow \argmin_{\theta_k} \mathbb{E} \left[ f(\theta_k; \mathbf{b}) \right] + \frac{\mu}{2} ||\theta_k - \theta^t_k||^2$\;
%         }
%     }
%     $\theta^{t+1}_k \leftarrow \theta^{t}_k$\;
%     \KwRet $\theta^{t+1}_{k}$\;
% }
% \end{algorithm}


